Depletion in post-AGB stars with a dusty disc. II

We present a chemical abundance analysis on the basis of high signal-to- noise and high resolution spectra for 12 stars of our newly defined sample. The selection criterion for the stars of this sample was their position in the `RV Tauri' box in the [12]-[25], [25]-[60] two-colour diagram. An additional requisite was the presence of a near-IR excess. We found that the photospheres of nine stars are affected by the depletion process. Since the most likely origin of the near-IR excess is a disc, this strongly suggests that the phenomenon of depletion and the presence of a disc are linked. Among the depleted stars we find different depletion patterns. In seven stars elements with a condensation temperature below 1500 K are not or only slightly affected. Large underabundances are measured only for most elements with a condensation temperature above 1500 K.

==> 1688aa <==
%% file: AAJOUR.BIB = journal strings, new AA & AoJ abbreviations
%% last: Oct 31 1995
%% baton: Rob Rutten, Sterrekundig Instituut Utrecht
%%     >> don't change this file - its baton is mine all the time <<

@STRING{acta = "Acta Astron."}
@STRING{actastsin = "Acta Astron.\ Sin."}
@STRING{actapsin = "Acta Astrophys.\ Sin."}
@STRING{advp = "Adv.\ Phys."}
@STRING{advsr = "Adv.\ Space Res."}
@STRING{amjp = "Am.\ J.\ Phys."}
@STRING{annap = "Ann.\ d'Astrophys."}
@STRING{annrev = "ARA\hbox{\rm \&}A"}
@STRING{araa = "ARA\hbox{\rm \&}A"}
@STRING{ao = "Appl.\ Opt."}
@STRING{appl = "Appl.\ Phys.\ Lett."}
@STRING{apb = "Appl.\ Phys.\ B"}
@STRING{afz = "Afz"}
@STRING{aa = "A\hbox{\rm \&}A"}
@STRING{aar = "A\hbox{\rm \&}AR"}
@STRING{aas = "A\hbox{\rm \&}AS"}
@STRING{agas = "Astron.\ Ges.\ Abstr.\ Ser."}
@STRING{aj = "AJ"}
@STRING{an = "Astron.\ Nachr."}
@STRING{azh = "AZh"}
@STRING{apj = "ApJ"}
@STRING{apjl = "ApJ"}
@STRING{apjss = "ApJS"}
@STRING{apss = "Ap\hbox{\rm \&}SS"}
@STRING{ap = "Astrophysics"}
@STRING{ajp = "Aust.\ J.\ Phys."}
@STRING{baas = "BAAS"}
@STRING{ban = "Bull.\ Astron.\ Inst.\ Neth."}
@STRING{bac = "Bull.\ Astron.\ Inst.\ Czech."}
@STRING{cjp = "Can.\ J.\ Phys."}
@STRING{cm = "Celest.\ Mech."}
@STRING{chinaa = "Chin.\ Astron."}
@STRING{cast = "Comments Astrophys."}
@STRING{fiz = "Fizika"}
@STRING{gafd = "Geophys.\ Astrophys.\ Fluid Dyn."}
@STRING{gj = "Geophys.\ J."}
@STRING{grl = "Geophys.\ Res.\ Lett."}
@STRING{geo = "Geophysics"}
@STRING{hd = "Hemel en Dampkring"}
@STRING{iauc = "IAU Circ."}
@STRING{iauib = "IAU Inf.\ Bull."}
@STRING{icarus = "Icarus"}
@STRING{jap = "J.\ Appl.\ Phys."}
@STRING{jaa = "JA\hbox{\rm \&}A"}
@STRING{jas = "J.\ Atmos.\ Sci."}
@STRING{jchemp = "J.\ Chem.\ Phys."}
@STRING{jcomp = "J.\ Comp.\ Phys."}
@STRING{jfm = "J.\ Fluid Mech."}
@STRING{jgr = "J.\ Geophys.\ Res."}
@STRING{jhast = "J.\ Hist.\ Astron."}
@STRING{jmolspec = "J.\ Mol.\ Spectrosc."}
@STRING{josa = "J.\ Opt.\ Soc.\ Am."}
@STRING{josaa = "J.\ Opt.\ Soc.\ Am.\ A"}
@STRING{josab = "J.\ Opt.\ Soc.\ Am.\ B"}
@STRING{jp = "J.\ Phys."}
@STRING{jpa = "J.\ Phys.\ A"}
@STRING{jpb = "J.\ Phys.\ B"}
@STRING{jpd = "J.\ Phys.\ D"}
@STRING{jpe = "J.\ Phys.\ E"}
@STRING{jpg = "J.\ Phys.\ G"}
@STRING{jpsj = "J.\ Phys.\ Soc.\ Japan"}
@STRING{jpp = "J.\ Plasma Phys."}
@STRING{jqsrt = "J.\ Quant.\ Spectrosc.\ Radiat.\ Transfer"}
@STRING{jrasc = "J.\ R.\ Astron.\ Soc.\ Can."}
@STRING{jetpl = "JETP Lett."}
@STRING{kfnt = "Kinematika Fiz.\ Nebesn.\ Tel"}
@STRING{msai = "Mem.\ Soc.\ Astron.\ Ital."}
@STRING{merc = "Mercury"}
@STRING{mag = "Mitt.\ Astron.\ Ges."}
@STRING{mn = "MNRAS"}
@STRING{mnras = "MNRAS"}
@STRING{mnassa = "Mon.\ Notes Astron.\ Soc.\ S.\ Afr."}
@STRING{nat = "Nat"}
@STRING{nature="Nat"}
@STRING{natwis = "Naturwissenschaften"}
@STRING{nattech = "Natuur en Techniek"}
@STRING{obs = "Observatory"}
@STRING{pfa = "Phys.\ Fluids A"}
@STRING{pfb = "Phys.\ Fluids B"}
@STRING{pla = "Phys.\ Lett.\ A"}
@STRING{plb = "Phys.\ Lett.\ B"}
@STRING{pra = "Phys.\ Rev.\ A"}
@STRING{prb = "Phys.\ Rev.\ B"}
@STRING{prc = "Phys.\ Rev.\ C"}
@STRING{prd = "Phys.\ Rev.\ D"}
@STRING{prl = "Phys.\ Rev.\ Lett."}
@STRING{ps = "Phys.\ Scr."}
@STRING{ptod = "Phys.\ Today"}
@STRING{pha = "Physica A"}
@STRING{phb = "Physica B"}
@STRING{phd = "Physica D"}
@STRING{pss = "Planet.\ Space Sci."}
@STRING{ppcf = "Plasma Phys.\ Controlled Fusion"}
@STRING{pasa = "Proc.\ Astron.\ Soc.\ Aust."}
@STRING{pi3e = "Proc.\ IEEE"}
@STRING{prsl = "Proc.\ R.\ Soc.\ London Ser.\ A"}
@STRING{posp = "Proceedings of SPIE"}
@STRING{pasj = "PASJ"}
@STRING{pasp = "PASP"}
@STRING{paspc = "PASPC"}
@STRING{qjras = "QJRAS"}
@STRING{ra = "Rev.\ Astron."}
@STRING{sciam = "Sci.\ Am."}
@STRING{sc = "Sci"}
@STRING{sky = "Sky Telesc."}
@STRING{sp = "Solar Phys."}
@STRING{sdb = "Soln.\ Dannye Byull."}
@STRING{sonne = "Sonne"}
@STRING{sa = "SvA"}
@STRING{sal = "SvA"}
@STRING{ssr = "Space Sci.\ Rev."}
@STRING{sf = "Spaceflight"}
@STRING{sterne = "Sterne"}
@STRING{sw = "Sterne Weltraum"}
@STRING{uao = "Upps.\ Astron.\ Obs.\ Rep."}
@STRING{va = "Vistas Astron."}
@STRING{zpa = "Z.\ Phys.\ A"}
@STRING{zpc = "Z.\ Phys.\ C"}
@STRING{zenit = "Zenit"}
@STRING{zetf = "Zh.\ Ehksp.\ Teor.\ Fiz."}
@STRING{ZsAp = "Zs.\ f.\ Ap."}
@STRING{ZsP = "Zs.\ f.\ Phys."}

